Are Machine Rationales (Not) Useful to Humans? Measuring and Improving Human Utility of Free-Text Rationales

Among the remarkable emergent capabilities of large language models (LMs) is free-text rationalization; beyond a certain scale, large LMs are capable of generating seemingly useful rationalizations, which in turn, can dramatically enhance their performances on leaderboards. This phenomenon raises a question: can machine generated rationales also be useful for humans, especially when lay humans try to answer questions based on those machine rationales? We observe that human utility of existing rationales is far from satisfactory, and expensive to estimate with human studies. Existing metrics like task performance of the LM generating the rationales, or similarity between generated and gold rationales are not good indicators of their human utility. While we observe that certain properties of rationales like conciseness and novelty are correlated with their human utility, estimating them without human involvement is challenging. We show that, by estimating a rationale's helpfulness in answering similar unseen instances, we can measure its human utility to a better extent. We also translate this finding into an automated score, GEN-U, that we propose, which can help improve LMs' ability to generate rationales with better human utility, while maintaining most of its task performance. Lastly, we release all code and collected data with this project.

==> sections/2_background.tex <==
\section{Analysis Setup}
\label{sec:analysis_setup}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/prompt_template.png}
    \caption{\textbf{Prompt templates for generating rationales:} Shown here are inputs and outputs of different template variations. Chain-of-Thought templates are taken from publicly released versions by \citet{cot}, whereas FEB and Fine-tuning templates are taken from \citet{marasovic-etal-2022-shot}.}
    \label{fig:prompt_template}
\end{figure*}

% \input{tables/prompt_templates.tex}

\paragraph{What is Human Utility?}
% \brihi{Update paragraph with new defition of utility considering I-O}
% We define human utility as the \textit{ability of a human to be able to solve the task correctly} \cite{idahl2021towards}. 
% It is shown that explainability methods are often used to debug models \cite{bhatt2019explainable} by practitioners, rather than facilitating trust between a model and a human.
% Note the difference between our definition of utility with that of forward simulation \cite{rigorous}. 
% Forward simulation requires a human prediction to match with that of the model, regardless of the true answer, and is more correlated with establishing trust between the model and the human.
We define human utility of rationales as \textit{the ability of a human to correctly solve a task with a rationale, that they are otherwise unable to} \cite{idahl-etal-2021-towards, chu2020arevisual}. 
% We can measure the human utility of a rationale \sahana{on the basis of} \textit{if the rationale helps the human solve the task correctly, when the human solves the task incorrectly without the rationale}.

More formally, let $\mathcal{F}$ be a \textit{self-rationalizing model} \cite{wiegreffe2020measuring} that can generate rationales with its predictions, and a corresponding input-output pair ${x, y}$.
$\mathcal{F}$ takes in $x$ as an input and generates a prediction $y_p$, and a rationale that corresponds to this prediction $r_p$.
The task accuracy (which corresponds to accuracy, when aggregated over all the instances) of this instance is given as follows: 
$$ \small \textsc{Task Accuracy} = \begin{cases} 
      1 & y_p = y \\
      0 & otherwise
   \end{cases}
$$

Let $\mathcal{H}$ be a human predictor that first takes in the instance $x$ and predicts a label for that instance, $y_h$.
Then, $\mathcal{H}$ is also shown the rationale $r_p$ and now takes both the instance and rationale ${x, r_p}$ as an input, and predicts a label $y_{hr}$.

Therefore, human utility of the rationale $r_p$ is calculated as:
$$ \small \textsc{Human Utility} = \begin{cases} 
      \textsc{Useful} & y_h \neq y\ and\ y_{hr} = y\\
      \textsc{Not Useful} & y_{hr} \neq y\\
      \textsc{Unsure} & y_h = y\ and\ y_{hr} = y
   \end{cases}
$$

In other words, rationales are \textit{useful} if a human incorrectly solved the task before, and with the introduction of the rationale, is able to correct their answer.
If even after being shown the rationale, the human is still solving the task incorrectly, this implies that the rationale has \textit{not} been useful.
However, if the human was correct both before and after being shown the rationale, we cannot conclusively determine the role of the rationale in helping solve the task.
We term these rationales are \textit{Unsure}.
These category of instances can either be too easy, or it can be the case that the human was already aware of the answer even before being shown the rationale. 
% \brihi{See if examples of unsure/useful/not useful rationales can be added to appendix}.
Of course, this can also imply that the rationale has still been useful in answering the task correctly, however, our definition of utility specifically evaluates cases where rationales are solely responsible for human utility.

% \subsection{Defining Utility Properties}
\paragraph{Task and Dataset Selection.}

We refrain from tasks used in existing free-text rationale works \cite{dataset_review} like NLI \cite{esnli} and Commonsense QA \cite{aggarwal-etal-2021-explanations}.
A primary reason for this is that humans are already able to reason better than models for NLI and Commonsense QA \cite{nangia2019muppet, talmor2021commonsenseqa}.
Therefore, the objective of machine rationales in this case is just to establish trust or generate faithful rationales. 
We aim to study rationale utility specifically in cases where the rationales can help with knowledge transfer that helps humans to correctly solve a task.
We thus impose the following constraints in our task and dataset selection:
\begin{itemize}
\setlength\itemsep{0em}
\item \textbf{Added advantage:} Tasks where machines can provide added advantage and that are not trivial or obvious for humans to solve.
\item \textbf{Objectivity:} Tasks where the reasoning has a limited scope of subjectivity.
% Tasks which are objective in nature, and where the reasoning has limited scope of subjectivity \sahana{What does `subjective' mean?}.
\item \textbf{Dataset size (of rationale annotations}): Size of gold rationales is considerably larger in the dataset, so as to provide room for training LMs with those rationales.
% \sahana{Do you mean to say dataset should have gold rationales?}.
\end{itemize}
In this work, we choose the StrategyQA dataset \cite{geva-etal-2021-aristotle}, which is an open-domain binary QA benchmark, where questions require implicit reasoning steps to be answered.
The StrategyQA dataset consists of an input question, the answer, along with intermediate implicit reasoning steps that are used to answer the questions. 
The implicit reasoning steps were generated by decomposing the original question into multiple questions. 
For our project, we combine these implicit reasoning steps and use them as rationales for a given instance. 

\paragraph{Self-rationalizing Models.}

\input{tables/finetuning_results.tex}


We try variations of in-context learning based approaches \cite{cot}, as well as few-shot and full finetuning approaches \cite{marasovic-etal-2022-shot} to generate rationales. 
For in-context learning based approaches, we vary the demonstrations based on the number of demonstrations desired, and the selection strategy for these demonstrations.
These demonstrations can either be fixed across all instances vs. randomly picked for each instance, from the training set.
Demonstrations that are picked randomly can either be six in number (to match a fixed number of demonstrations as per \citet{cot}), or determined by a maximum token length that is specific beforehand (for our experiments, we use $2048$ as the maximum token length of an input).
For these settings, we implement two input-output templates -- where rationales $r_p$ come after (FEB) \cite{marasovic-etal-2022-shot} or before the prediction $y_{hr}$ respectively (Chain-of-Thought or CoT) \cite{cot}. 
The LM used for all in-context learning experiments is GPT-3 \cite{gpt3}.
For fine-tuning approaches, we fine-tune two LMs - T5 \cite{t5} and UnifiedQA \cite{khashabi-etal-2020-unifiedqa}, with varying sizes - large and 3B. 
For each of these two LMs, we use four variations of input-output templates (SQuAD-T5, Infilling, T5-Like and QA-simple), as defined by \citet{marasovic-etal-2022-shot}. 
Examples of each of these templates are provided in Figure \ref{fig:prompt_template}. 

\input{tables/incontext_results.tex}

As seen in Tables \ref{tab:icl_res} and \ref{tab:finetune_res}, for the StrategyQA dataset, FEB templates with randomly selected demonstrations provides the highest accuracy for in-context learning approaches, whereas the infilling template consistently outperforms other input-output templates for fine-tuning approaches.
For the rest of our work, we select three best performing LM configurations with varying sizes -- (1) GPT-3 (with FEB template, and 6 randomly selected demonstrations), (2) T5-large (with infilling template, fine-tuned on the entire training set) and (3) T5-3B (with infilling template and 128-shot fine-tuning).

==> sections/3_rq1.tex <==
\section{Does Task Performance Correlate with Human Utility?}
\label{sec:perf_util}
% \brihi{Update results w.r.t new definition of utility with I-O control case.}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/properties.png}
    \caption{\textbf{Granular-level Rationale Properties: }Definitions for properties along each axes (surface form, informativeness, support and style) are shown. For all but style axes, an example of a rationale \textit{satisfying} the property is also shown. For style, we show examples of rationales that do not satisfy the given properties.}
    \label{fig:properties}
\end{figure*}

\paragraph{Task Performance.} For the three selected best performing LM configurations, we note (Tables \ref{tab:icl_res}, \ref{tab:finetune_res}) that task performance increases after the LM is forced to generate rationales. 
This is also consistent with prior findings \cite{cot, marasovic-etal-2022-shot}.

\paragraph{Human Utility Annotations.} We conduct human-subject studies to evaluate utility of free-text rationales. 
For each StrategyQA test instance, we ask humans to first provide an answer given the question.
We then show them a rationale and ask them to answer the question again.
The rationale shown to them is generated by either of the three selected LMs.
We use Amazon Mechanical Turk \footnote{\href{www.mturk.com}{www.mturk.com}} to first curate a set of annotators that understand the task well (via extensive qualification tests). 
Each instance is answered by five annotators.

We observe that, StrategyQA instances are difficult to annotate by humans, as a lot of them are fact-based, which the human might or might not know beforehand.
Therefore, human agreement before the rationale is shown is low (Krippendorf's $\alpha=0.18$). 
However, after being shown the rationale, the agreement increases, with Krippendorf's $\alpha$ being $0.47$, $0.30$ and $0.24$ for GPT-3, T5-3B and T5-Large LMs respectively.
Examples of rationales annotated into each of the three human utility categories (useful, not useful, unsure) is in the Appendix (Table \ref{tab:examples_utility}).

% \brihi{Add table of human perf before and after rationales}

\paragraph{Correlation between Task Performance and Human Utility.}
For each instance, we calculate human utility as defined in \textsection \ref{sec:analysis_setup}, where predictions made by five annotators are aggregated by taking a majority vote.
% For each instance, we pick the majority vote \sahana{majority vote of what?} as the final label. 
Overall, while including annotations for all models combined, we observe that the correlation between task accuracy (whether a given instance was correctly predicted by the self-rationalizing model) and human utility of a rationale (useful, not useful and unsure) was close to none (Theill's $U = 0.0359$). 
This indicates that while generating rationales might improve overall task performance, there is no guarantee that these rationales useful for humans in solving the task correctly. 

In fact, if we look at the correlations for each LM separately, we observe Theill's $U$ for GPT-3, T5-3B and T5-Large were $0.111$, $0.034$ and $0.005$ respectively. 
This also demonstrates that even though T5-Large, which was fine-tuned on the entire training set had the highest task performance, it has the lowest correlation with human utility.

==> sections/4_rq2.tex <==
\section{What are the Properties of Rationales that are Useful?}
\label{sec:properties}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/properties.png}
    \caption{\textbf{Granular-level Rationale Properties: }Definitions for properties along each axes (surface form, informativeness, support and style) are shown. For all but style axes, an example of a rationale \textit{satisfying} the property is also shown. For style, we show examples of rationales that do not satisfy the given properties.}
    \label{fig:properties}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/properties_splitted_analysis.png}
    \caption{\textbf{Distribution of Property Annotations for Different Rationales:} Distribution is generated by aggregating scores of five annotators of each instance. A higher value implies more presence of the property in the rationale generated by the particular LM.}
    \label{fig:properties_distribution}
\end{figure*}

% \brihi{Fix Results and Property Descriptions}
As we have observed in \textsection \ref{sec:perf_util}, higher task performance does not necessarily correlate with the rationales being useful for humans in solving the task.
We follow up this discussion by investigating more granular-level properties that associate with human utility of rationales.
% \sahana{high utility for humans?}.

\paragraph{Granular-level Rationale Properties.} 
% \brihi{Add citations for properties either here or in related work}
What are some granular-level properties of rationales that are useful? 
Can such qualities help distinguish between rationales that are useful, to those that are not useful or ones we are unsure about?
To answer the above questions, we follow list a set of desirable properties of that useful rationales should satisfy \cite{wiegreffe-etal-2021-measuring, wiegreffe-etal-2022-reframing, roscoe}.
These properties evaluate rationales along four axes - surface form qualities, support towards predicted labels, informativeness and style. 
Surface form qualities test whether a rationale is \textit{grammatical} and \textit{factually valid}. 
\textit{Association} with label and \textit{contrast} between different labels measure the extent to which rationales support the labels that were generated with them.
We also evaluate the informativeness of a rationale, which is determined by \textit{novel information} that the rationale provides over the question, along with asking whether it directly \textit{leaks the answer}.
Lastly, we also check whether the rationale contains \textit{irrelevant hallucinations} or relevant but \textit{redundant information}.
Descriptions and examples of these properties are shown in detail in Figure \ref{fig:properties}.

% \brihi{Ziyi to add reference to properties figure}
\paragraph{Human Annotations.}

For rationales generated by all three LMs, as well as gold rationales, we conduct human studies to evaluate whether the rationales satisfy the given properties.
For each instance, a property is marked on a binary scale (Yes / No), indicating the presence or absence of that property and evaluated by five annotators. 
Each category of properties is evaluated on a separate HIT, for which instructions have been modified so as to ensure that the annotators understand our definitions of the properties.
Given the complex nature of the human study, we make sure that the property annotations reach low to moderate agreement across all annotators (Appendix \ref{tab:property_annotation_agreement}).
% \brihi{Add agreement rate numbers}.

\paragraph{Property Analysis.}

We first study the presence of these properties in rationales, without considering the utility of these rationales.
Figure \ref{fig:properties_distribution} plots the distribution of these properties, split by the models that generate these rationales, along with Gold rationales.
The distributions are obtained by taking the mean of ratings from five annotators for a given instance, where a higher value indicates a more frequent presence of that particular property in the set of rationales.
We observe that Gold rationales, in comparison to other model-generated rationales, have lower scores for leakage and higher scores for other properties.
In fact, Gold rationales are always associated with the gold label, which serves as a sanity check, as they are designed to help answer the gold label.
% \sahana{move sanity check to the end of the sentence.}
While all types of rationales are mostly grammatically correct
% \sahana{(change to) grammatically correct (also point to corresponding scores in table)}
, T5-large and T5-3B suffer at producing rationales that are factually correct, and T5-large 
T5-large rationales also tend to hallucinate and produce redundant sentences in rationales more often. 
% \sahana{In some places you say `the rationales' in the passive voice, and in other places you say `T5 produces rationale that is' in active voice. It might be good to standardize this across the whole paper.}
While GPT-3 rationales tend be generally better than T5-large and T5-3B for surface-form and stylistic properties, they leak the predicted label more often than them. 
There is high variation for rationale-label association and contrasting features in rationales for all model-generated rationales, however on average, GPT-3 generated rationales are better on these metrics too. 
% \sahana{Point to some table/corroborating scores in all these sentences.}

\paragraph{Properties of Useful Rationales. }
% To Add - 
% 1. GLMER modelling
% 2. Cite QED and other paper, including R libraries
% 3. Tell about properties which lead to higher increase in log odds of utility
% 4. Talk about pairs of properties that have the highest increase in utility from base --> add table

We use a Generalized Linear Mixed-Effects Model (GLMEM) (similar to \citet{lamm2020qed}) to model the correlation of different properties and their interactions with that of high utility. 
The formula used for modelling the GLMEM is as follows: 
$ \small \textsc{Response} = (\textsc{Grammaticality} + \textsc{Validity} + \textsc{Coherence} + \textsc{Conciseness} + \textsc{Leakage} + \textsc{Novelty} + \textsc{Association} + \textsc{Contrast})^2 + (1|\textsc{Question ID}) + (1|\textsc{Model ID}) + (1|\textsc{Human Prior})$

The response (dependent variable) is human accuracy after the human was shown the rationale. More formally,
$$ \small \textsc{Response} = \begin{cases} 
      1 & y_{hr} = \hat{y}\\
      0 & y_{hr} \neq \hat{y}\\
   \end{cases}
$$
All properties, along with their second-order interactions (implemented using the squared term above) are dependent variables.
Furthermore, we try to control for random effects whose variability might influence the response.
We control for randomness induced by a particular question, the model generating the rationales or whether the human had correctly answered the question before (Human Prior). More formally,
$$ \small \textsc{Human Prior} = \begin{cases} 
      1 & y_{h} = \hat{y}\\
      0 & y_{h} \neq \hat{y}\\
   \end{cases}
$$

\input{tables/property_individual.tex}

Table \ref{tab:property_individual} shows the log odds of a rationale being useful, when a certain property is present or absent, while averaging over other properties.
We note that all of the log odds are negative, which means that in isolation, the presence or absence of any property is does not correlate well with rationales of high utility.

\input{tables/properties_pair.tex}

We then look at pairwise interactions. 
Table \ref{tab:property_interactions} shows top ten pairs which lead to an increase in utility log odds from the base level (Intercept), which is when a rationale does not satisfy any property.
A grammatically correct rationale that explicitly leaks the answer leads to the highest increase in log odds. 
This is also intuitive, as leakage is a direct signal to a human to select a given answer, without any reasoning from the human's behalf.

When all possible combinations of properties are considered, presence of all but coherence and association leads to a positive log odds for rationale utility: $0.139$. 
This implies that humans are generally robust to hallucinations that are irrelevant to the question.
Furthermore, association of the rationale with its predicted label is also not an important property for rationale utility, as the rationale may not be associated with the correct answer and therefore, mislead the human into making an incorrect choice.






==> sections/5_rq_gen.tex <==
\section{Can Rationales with High Utility Help Humans Generalize to New Instances?}
\label{sec:generalization}

\input{tables/generalization_examples.tex}

As we have defined and shown in previous sections, human utility of rationales is determined by their ability to guide humans to correctly solve tasks.
We follow this up by investigating if humans can generalize to syntactic or semantic perturbations of the original question, while being shown rationales of the original question.
This will help us understand if human utility of rationales can also indicate whether rationales help with knowledge transfer for unseen instances.
% \brihi{Add intro paragraph}.
% \brihi{Need to find citations for human generalization to new instances}.
% \sahana{Can you add a line saying what you mean by `Useful' rationales? Do you mean the rationales which you found had human utility in Section 3?}
% \sahana{Do you mean that the new instances use the same rationale (i.e., the rationale that was found to have utility)? I think you should clarify why this section is relevant.}
\paragraph{Types of Generalization Questions.}

For our study, we consider three distinct types of generalization setups. 
Firstly, we evaluate the human $\mathcal{H}$'s ability to generalize to non-trivial \textbf{rephrases} of the original question.
% These instances are non-trivial rephrases of the original question. 
We avoid simple rephrases like changing a preposition, or removing an adverb so as to avoid near duplicates of the original question.
Next, we look at \textbf{counterfactual} questions. 
These questions follow the same reasoning steps of the original question, however, they flip the answer of the original question. 
Lastly, we test $\mathcal{H}$'s ability to understand questions that follow a \textbf{similar reasoning} process as the original question, but are not related to the original question.
These questions can entail entity swaps, or questions that uses one of the reasoning steps to answer the original question.
% \brihi{Add generalization examples table}
Examples of each type of generalization question is shown in Table \ref{tab:generalization_examples}.

\paragraph{Generating Generalization Questions.} 

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/generalization.png}
    \caption{\textbf{Generating Generalization Questions:} A question, rationale, answer triplet is fed to GPT-3 using given templates. GPT-3 generates potential generalization question candidates from each template, which are then manually filtered and answered to create gold labels in-house.
    \xiang{Probably need to compress for saving space. We can minimally just show the questions alone, and leave others to appendix.}
    }
    \label{fig:generalization_pipeline}
\end{figure*}

For generating generalization questions as describe above, we follow the Human and AI collaboration paradigm as introduced by \citet{wanli}.
% \brihi{Confirm number of demonstrations and types for each category from Ziyi.}
We first start by manually creating templates with instructions for each type of generalization question.
We then select six demonstrations for these templates.
The selected instructions and demonstrations are in Appendix (Table \ref{tab:generalization_demonstrations}).
These demonstrations are fixed for each type (however, may differ across the different types) and are selected from the training set.
% \brihi{Add figure ref}
For every test instance, we insert it at the end of the corresponding template, which is then used as a prompt for GPT-3 to generate questions. 

We then manually filter the generated questions in-house and provide gold answers for them, to make sure that the final set of questions are of good quality.
Finally, we have a set of $123$ rephrase, $102$ counterfactual and $171$ similar reasoning generalization questions that are of good quality from the test set.
The pipeline and examples of the templates are shown in Figure \ref{fig:generalization_pipeline}.

\paragraph{Human Annotations.} 

Similar to \textsection \ref{sec:perf_util}, we first ask the annotators to answer a given question with and without the rationale.
We then show them a generalization question, which they have to answer while referencing the rationale for the original question. 
We repeat the experiment above with rationales from the three LMs, along with gold rationales.
Each instance is annotated by five annotators.
Given that there are no corresponding rationales for the generalization questions, this annotation setup would measure the impact of rationales of the original question towards answering the generalization questions.
% \sahana{Ok, you have answered my previous note here. It might be worth adding a small note about this over there as well?}

\paragraph{Results.}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/generalization_results.png}
    \caption{\textbf{Generalization Performance:} Shown here is generalization accuracy for different generalization question types, split by LM-generated and gold rationales. The \textit{Combined} group is aggregated across all LM-generated rationale performance. }
    \label{fig:generalization_results}
\end{figure*}

Figure \ref{fig:generalization_results} shows generalization accuracy of rationales with different human utility, split across different LM's generating them as well as gold rationales.
We observe that gold rationales form an upper bound for generalization accuracy, across all types of generalization questions and types of rationale utility.
Useful rationales are always significantly better than non-useful rationales while answering generalization questions, which indicates that rationale utility is a strong signal for generalizing to newer instances.
Paraphrases of original questions are relatively easier to answer, when compared to counterfactuals and similar reasoning, as it can be seen by both Gold rationale, as well as accuracy of all models combined.
We can also note that GPT-3 generated rationales help generalize better to more difficult scenarios like counterfactuals or similar reasoning questions.
Rationales that we are unsure of in terms of utility are helpful in generalizing to paraphrases or similar reasoning questions.
This indicates the presence of easy-to-answer questions in that bucket of instances, which also hints towards the fact that their paraphrases or similar reasoning counterparts would also be easier to answer. 
% \sahana{Can you rephrase this sentence? I don't understand it.}
Counterfactuals however show a different trend, where unsure rationales have a lower generalization accuracy when compared to useful rationales. 
Examples of generalization questions which were answered correctly/incorrectly for rationales that have high or low human utility is shown in the Appendix (Table \ref{tab:generalization_utility_examples}).

==> sections/abs_old.tex <==
% \renewcommand{\brihi}[1]{}
% \renewcommand{\ziyi}[1]{}
% \renewcommand{\zhewei}[1]{}
% \renewcommand{\aaron}[1]{}
% \renewcommand{\ameya}[1]{}
% \renewcommand{\sahana}[1]{}
% \renewcommand{\xiang}[1]{}


% State-of-the-art language models (LMs) can be trained or prompted to generate fluent text for solving various NLP tasks.
% \brihi{Need to restructure better after feedback}
% State-of-the-art language models (LMs) can be finetuned or prompted to explain their own decisions by generating free-text rationales
% State-of-the-art language models (LMs) have been shown to improve downstream task performance while generating fluent free-text rationales or chains-of-thought that explain their predictions.
Recently, there has been growing interest in using language models (LMs) for human-AI collaboration.
To explain their reasoning processes to humans, state-of-the-art LMs have been shown to fluently generate free-text rationales (FTRs), \eg via chain-of-thought prompting. 
% State-of-the-art language models (LMs) have been shown to improve their downstream task performance by jointly generating free-text rationales to explain their task predictions.
% This ability has also paved way to prompt these LMs to generate free-text rationales explaining their decisions. 
% While jointly generating task outputs and free-text rationales may improve LMs' task performance, it is unclear how useful these LM-generated rationales actually are to human users.
% Although these LM-generated rationales may appear fluent, it is often unclear how useful they are to humans.
% However, there is no guarantee that these generated rationales are actually helpful to humans in understanding the task.
Still, it remains unclear how effectively these generated FTRs can provide \textit{human utility} for human-AI collaboration, \ie assist humans in solving NLP tasks.  
% \xiang{should add a 2nd sentence in abs to speak out “why we care human utility” besides other use of the FTRs.}
% In this work, we ask: can these rationales also contribute to \textit{improving human utility} of accomplishing a given task?
% To investigate this, our paper studies four questions: (1) To what extent do generated rationales provide utility to humans for solving NLP tasks? (2) What is the relationship between generated rationales' human utility and the LM's task performance? (3) Which properties of generated rationales are most positively correlated with human utility? (4) Can useful rationales help humans generalize to new instances?
% \aaron{RQ4 is kind of confusing, since it's unclear what "useful rationales" are at this point. Before we introduce the four RQs, we should probably first define (at a high-level) what utility is, since this definition is a critical part of our paper}
% \ziyi{"Can rationales be generalizable to new instances?"}
% In this work, we investigate the association between an LM's task performance, and the human utility of rationales generated by these LMs. 
% We define utility as the ability of a human in being able to solve the task or generalise to new instances of the task, when being shown the machine rationale.
% To investigate this, we deem rationales to have high human utility if they can \textit{guide} humans to correctly solve a task that they are otherwise unable to.
% RQ1
% \aaron{Seems like the finding for RQ1 is missing} -- % Brihi: There seems to be a mistmatch as we arent really doing RQ1. I will have to remove it
% RQ1
% By comparing three LMs with different rationale-generation techniques \aaron{This sounds like the rationale generation strategies are tools for comparing the LMs. I don’t think this is what you mean? I thought we are trying to compare the rationales, which can be obtained via different types of LMs and generation strategies. Also, the description of this setting can be decoupled from the RQ findings}, we find that task performance has no correlation with the human utility of rationales in actually solving the task, and larger LMs like GPT-3 generate rationales that are more useful to humans in solving the task, as compared to relatively smaller LMs like T5, even though the latter yields better task performance \aaron{This sentence is too long/unclear. GPT-3 vs. T5 part should be its own sentence, but not so detailed (\eg remove LM names). Why not just say something like: LM size is more positively correlated with human utility, while finetuning is more important for task performance?}.
To investigate what makes an FTR useful to humans, this paper analyzes the relationships between human utility and various LM/FTR properties.
First, although LMs are often finetuned/prompted to jointly generate task labels and FTRs, we find that LMs' task performance has little correlation with human utility, whereas LM size is a positive predictor of human utility.
% Meanwhile, LM size and LM finetuning are positive predictors of human utility and task performance, respectively.
% We find that downstream task performance is not correlated with human utility of rationales.
% In fact, LM size is a better indicator of human utility, while higher task performance is achieved on finetuning smaller LMs.
% RQ2
% Furthermore, we find that while individually properties like grammar, factual correctness, novelty, prediction label leakage, rationale-label association, label-contrast as well as stylistic properties like coherence and conciseness are not correlated with an increase in rationale utility, all but association and coherence combined together can lead to an increase in human utility of rationales \aaron{Unclear what a lot of these properties mean. Can we only include the minimum (and most self-explanatory) info needed to summarize this finding? That is, rather than simply listing that Properties [1-8 / 9-10] are [negatively / positively] correlated with rationale utility, why not summarize the broader lessons that we learn from these results? What do Properties 1-8 have in common? What do Properties 9-10 have in common? How do these commonalities relate to rationale utility? All of this needs to be distilled into 1-2 sentences.}. \sahana{Perhaps you can use `surface form qualities, support towards predicted labels, informativeness and style' - you have used these in Section 4 and they summarize the list of properties well.}
% Second, we observe that individual FTR properties (\eg conciseness, novelty) are not predictive of human utility, while the presence of certain property pairs (\eg conciseness+novelty) is a strong positive predictor of human utility.
Second, we observe that certain FTR property pairs are strong positive predictors of human utility, \eg high-utility FTRs tend to both be concise and contain novel information.
% Furthermore, our findings also show that high utility rationales are often informative and concise, while also supporting LMs' decisions. 
% RQ3
% Lastly, we observe that useful rationales \aaron{What does useful mean here? Seems like generalizability is also an aspect of usefulness?} can help humans generalize to new instances (like rephrases or counterfactuals of original instances, as well as instances which follow a similar reasoning process \aaron{Too wordy/detailed. Need to compress}) much better \aaron{Why is this true? Why does this matter?}, as compared to rationales that are not useful for humans \aaron{Redundant}.
Third, we show that high-utility FTRs for a given task instance can provide transferable knowledge that helps humans generalize to solving new instances.
% We also observe that a high utility rationale for a given instance contains enough context to help humans generalize to even unseen instances, for which they do not have access to any rationales.
By shedding light on the nature of FTRs' human utility in practical settings, our findings can help guide future work on designing LMs and FTR generation strategies for stronger human-AI collaboration.

% We believe that investigating human utility of rationales can better situate LMs in real-world scenarios, where human-LM collaboration is required to improve both human understanding of the task as well as LM performance.
% \aaron{We aren't emphasizing the human-AI collaboration aspect at all in the abstract/intro (and rest of paper?). Need to make this the core motivation for the work}
% Points for abstract:

% 1. Free-text rationale generation from LMs
% 2. Task improvement via rationalisation
% 3. human utility and understanding of these rationales are not clear. Often not good rationales
% 4. Findings about human utility
% 5. Property correlations with human utility
% 6. Generalization 


==> tables/prompt_templates.tex <==
\begin{table*}[h!]
\centering
\scalebox{0.60}{
\begin{tabular}{ccll}
\toprule
\textbf{Method Type} & \textbf{Template} & \multicolumn{1}{c}{\textbf{Input}} & \multicolumn{1}{c}{\textbf{Output}} \\
\midrule
\multirow{11}{*}{In-Context Learning} & Chain-of-Thought & \begin{tabular}[c]{@{}l@{}}\emph{Q:} \colorbox{lyellow}{Demonstration Question 1}\\ \emph{A:} \colorbox{pink}{Demonstration Rationale 1}. The Predicted Answer is \\ \colorbox{lgreen}{Demonstration Answer 1}.\\ .... (repeated based on $\#$ of demonstrations)\\ \emph{Q:} \colorbox{lyellow}{Input Question}\\ \emph{A:}\end{tabular} & \colorbox{pink}{Generated Rationale}. The answer is \colorbox{lgreen}{Predicted Answer}. \\
\cmidrule(lr){2-4}
 & FEB & \begin{tabular}[c]{@{}l@{}}\emph{Answer the Input Question from the provided choices,} \\ \emph{and provide a reason why the Predicted Answer is correct.}\\ \emph{Question:} \colorbox{lyellow}{Demonstration Question 1}\\ \emph{Choices:} Yes or No\\ \emph{Answer:} \colorbox{lgreen}{Demonstration Answer 1}\\ \emph{Reason:} \colorbox{pink}{Demonstration Rationale 1}\\ .... (repeated based on $\#$ of demonstrations)\\ \emph{Question:} \colorbox{lyellow}{Input Question}\\ \emph{Choices:} Yes or No\\ \emph{Answer:}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\colorbox{lgreen}{Predicted Answer}.\\ \emph{Reason:} \colorbox{pink}{Generated Rationale}\end{tabular} \\
\midrule
\multirow{8}{*}{Fine-tuning \\} & SQuAD-T5 & \begin{tabular}[c]{@{}l@{}}\emph{explain strategyqa Input Question:} \colorbox{lyellow}{Input Question}\\ \emph{context:} True, False\end{tabular} & \colorbox{lgreen}{Predicted Answer} because \colorbox{pink}{Generated Rationale}. \\
\cmidrule(lr){2-4}
 & Infilling & \begin{tabular}[c]{@{}l@{}}\emph{explain strategyqa Input Question:} \colorbox{lyellow}{Input Question} \\ \emph{choice:} True, False  <extra\_id\_0> because <extra\_id\_1>\end{tabular} & \begin{tabular}[c]{@{}l@{}}<extra\_id\_0> \colorbox{lgreen}{Predicted Answer} <extra\_id\_1>\\ \colorbox{pink}{Generated Rationale} <extra\_id\_2>\end{tabular} \\
 \cmidrule(lr){2-4}
 & T5-Like & \begin{tabular}[c]{@{}l@{}}\emph{explain strategyqa query:} \colorbox{lyellow}{Input Question}\\ \emph{entities:} True, False\end{tabular} & \colorbox{lgreen}{Predicted Answer} because \colorbox{pink}{Generated Rationale}. \\
\cmidrule(lr){2-4} 
 & QA-simple & \emph{explain}\colorbox{lyellow}{Input Question} \emph{A) True B) False} & \colorbox{lgreen}{Predicted Answer} because \colorbox{pink}{Generated Rationale}. \\
\bottomrule
\end{tabular}}
\caption{\textbf{Prompt templates for generating rationales:} Shown here are inputs and outputs of different template variations. Chain-of-Thought templates are taken from publicly released versions by \citet{cot}, whereas FEB and Fine-tuning templates are taken from \citet{marasovic-etal-2022-shot}.}
\label{tab:prompt_templates}
\end{table*}
